Uncertainty Quantification of Spatiotemporal Travel Demand with Probabilistic Graph Neural Networks

Recent studies have significantly improved the prediction accuracy of travel demand using graph neural networks. However, these studies largely ignored uncertainty that inevitably exists in travel demand prediction. To fill this gap, this study proposes a framework of probabilistic graph neural networks (Prob-GNN) to quantify the spatiotemporal uncertainty of travel demand. This Prob-GNN framework is substantiated by deterministic and probabilistic assumptions, and empirically applied to the task of predicting the transit and ridesharing demand in Chicago. We found that the probabilistic assumptions (e.g. distribution tail, support) have a greater impact on uncertainty prediction than the deterministic ones (e.g. deep modules, depth). Among the family of Prob-GNNs, the GNNs with truncated Gaussian and Laplace distributions achieve the highest performance in transit and ridesharing data. Even under significant domain shifts, Prob-GNNs can predict the ridership uncertainty in a stable manner, when the models are trained on pre-COVID data and tested across multiple periods during and after the COVID-19 pandemic. Prob-GNNs also reveal the spatiotemporal pattern of uncertainty, which is concentrated on the afternoon peak hours and the areas with large travel volumes. Overall, our findings highlight the importance of incorporating randomness into deep learning for spatiotemporal ridership prediction. Future research should continue to investigate versatile probabilistic assumptions to capture behavioral randomness, and further develop methods to quantify uncertainty to build resilient cities.

==> backup.tex <==
\title{Uncertainty Quantification of Spatiotemporal Travel Demand with Graph Convolutional Neural Networks}

\author{Qingyi Wang, Shenhao Wang\footnote{Corresponding Author; Email: shenhao@mit.edu}, Haris Koutsopoulos, Jinhua Zhao}


% As a general rule, do not put math, special symbols or citations
% in the abstract or keywords.
\begin{abstract}
Uncertainty prevails in transport systems. Although recent studies adopted deep learning to predict the spatiotemporal patterns in travel demand, they largely ignored the spatiotemporal structure of the demand uncertainty. This study designs a truncated mean-variance estimation (TMVE) method for the Graph Convolutional Long Short Term Memory neural network (GCN), simultaneously estimating the mean and variance to quantify the spatiotemporal uncertainty in travel demand. Our experiments target the prediction of the mean-variance structure of rail demand in Chicago. The TMVE-GCN model exhibits significant improvements in the estimation of prediction intervals without sacrificing the quality of the mean prediction. The model also has high generalizability: it performs effectively on not only the pre-COVID data, but also the data at the COVID recovery stage, despite the drastic demand change caused by COVID-19. The spatiotemporal variance of the rail demand presents patterns similar to the mean values: demand uncertainty is most significant during the rush hours and at high demand stations. Overall, this study expands the deep learning-based travel demand analysis by quantifying uncertainty, develops innovative methods to describe the spatiotemporal uncertainty structure, and empirically demonstrates the spatiotemporal uncertainty patterns for rail ridership. Future studies can expand this research by comparing the TMVE-GCN method to other algorithms and using the uncertainty structure to inform the design of resilient transportation systems.  
\end{abstract}
%\cite{Abdar2020}
\section{Introduction}
The recent literature is paying an increasing attention to the short-term demand prediction with prediction horizons from five minutes to a couple of hours, which is enabled by the smart devices on vehicles providing data with high time and space resolution. The accurate prediction of the short-term demand can help with the decision-making and assessment of short-term planning and control strategies. At the same time, this is a challenging problem that involves high uncertainty and complex spatiotemporal relationships. Traditionally, time series and spatial-lag models were used. In recent years, deep learning has achieved impressive performance in lowering the prediction error by leveraging temporal information with long short term memory networks and spatial information with convolutional or graph convolutional networks. However, despite some recent efforts \cite{Rodrigues2020}, researchers mainly focused on the prediction of average demand through the deep learning framework, but largely ignored the uncertainty structure inevitably associated with any demand prediction. Overlooking the prediction uncertainty leads to both theoretical and practical problems. First, when the error structure is not taken into account, models inherently assume constant variance (homoskedasticity). This assumption has been challenged and shown empirically as invalid \cite{Yang2019}. Second, while a point prediction provides a valuable baseline for system design and operations, it is widely acknowledged in the decision-making literature that, predictive uncertainty is unavoidable and valuable for building systems more robust to day-to-day variations of demands and minor disruptions. An abundance of literature in robust service planning that make use of uncertainty estimates in projected demand has shown superior performance compared to benchmark models with mean estimates only \cite{Kumar2018,Li2015,Ukkusuri2007}. For example, while making rebalancing decisions for mobility-on-demand services, it is shown that taking demand uncertainty into account would reduce customer wait times in the system \cite{Guo2021}.

This study, therefore, challenges the homoskedasticity assumption and quantify the predictive uncertainty in deep learning for short-term transit demand prediction using data from the Chicago Transit Authority (CTA). To quantify the spatiotemporal uncertainty, a model with a heteroskedastic error is proposed using the truncated mean-variance estimation in a graph convolutional long short term memory network (TMVE-GCN). The magnitude and patterns of uncertainty are then studied and compared with those from the benchmark models. Lastly, model generalizability is tested against time shifts with substantial demand changes (pre- and post-COVID periods). The contributions of this study are
\begin{enumerate}
    \item Showing the existence of heteroskedasticity in travel demand.
    \item Designing a deep-learning-based algorithm to quantify travel demand uncertainty that outperforms benchmark models.
    \item Interpreting the spatiotemporal uncertainty patterns of travel demand. 
    \item Demonstrating model generalizability for pre- to post-COVID periods
\end{enumerate}


\section{Literature Review}
\subsection{Prediction with Deep Learning in Transportation}
In recent years, researchers have made significant progress in applying deep learning to forecast travel demand, both on the individual decision-making level \cite{Wang2019,Wang2019a,Zhao2018} and aggregate trip count level \cite{NoursalehiDynamicApproach, Liu2018UrbanLearning}. The most common method is the class of Convolutional LSTM (CNN-LSTM) models because of their capacity in capturing the spatiotemporal travel demand patterns. The examples of the CNN-LSTM models used in travel demand predictions include the diffusion convolutional recurrent neural network (DCRNN) to predict traffic flows \cite{Li2018DiffusionForecasting}, CNN and LSTM models to forecast taxi demand \cite{Yao2018DeepPrediction}, and spatiotemporal residual neural networks (ST-ResNet) for citywide crowd flows in Beijing and NYC \cite{Zhang2017DeepPrediction}. CNN is designed to analyze quantities on an urban grid, and convolutions are defined with respect to neighbouring cells on an imposed artificial grid. Due to the graph nature of some urban structures, such as transit lines, correlations may not be defined by immediate surroundings, but rather upstream and downstream stops. As a result, graph neural networks (GNN) and their variants are better suited to problems with a graph structure, since convolutions are defined by adjacency relationships on graphs \cite{Ye2020HowSurvey}. For example, a spatiotemporal multi-graph convolution network (ST-MGCN) was used to predict ride-hailing demand \cite{Geng2019SpatiotemporalForecasting} and inflows and outflows at transit stations \cite{Han2019PredictingNetworks,Ye2020Multi-STGCnet:Forecasting}, combined GNN and RNN was used to predict parking occupancy at the block level \cite{Yang2019ASources}, and metro ridership for multiple time periods \cite{Liu2020Physical-VirtualPrediction}. However, existing models produce only the expected value of travel demand. To characterize a random quantity such as travel demand, uncertainty estimates in the form of variance and/or quantiles are needed. 

\subsection{Uncertainty Quantification Framework}\label{uncertainty_framework}
In the uncertainty quantification literature, researchers typically differentiate between data (aleatoric) and model (epistemic) uncertainty \cite{Kiureghian2009AleatoryMatter}, and their sum is referred to as prediction uncertainty. Using a simple regression formula $y_i = f(x_i) + \epsilon_i$ as an example, the model uncertainty $\sigma_{model}^2$ refers to the uncertainty resulting from the difference between $f(x_i)$ and the estimated $\hat{f}(x_i)$, the data uncertainty $\sigma_{data}^2$ refers to the error term $\epsilon_i$ inherent in the data generating process, and the prediction uncertainty describes the overall difference between the actual $y_i$ and the predicted $\hat{y_i}$. Their relationship is given by $\sigma_y^2 = \sigma_{model}^2 + \sigma_{data}^2$. Model and data uncertainty stems from different factors. Three factors that could explain model uncertainty are: (1) limitations of model functional form - the discrepancy between $\hat{f}$ and $f$ given enough training data; (2) sampling – since the training set is only a sample of the population, different samples give different model estimations; (3) parameter identification - deep learning models are overparameterized and converge to different local minima with different initializations, where the stability of the estimated parameters largely depends on sample size \cite{Pearce2018High-qualityApproach}. On the other hand, data uncertainty results from unavailable explanatory factors and unavoidable random noise in the data, and is therefore often referred to as irreducible uncertainty. 

Different algorithms have been developed to quantify both types of uncertainty. In particular, forward uncertainty quantification algorithms are designed to quantify data uncertainty and inverse uncertainty quantification algorithms calibrate models post-estimation to quantify model uncertainty. Several review papers have been written on the advantages and disadvantages of the forward and inverse uncertainty quantification algorithms \cite{Tibshirani1996AModels, Papadopoulos2001ConfidenceComparison,Kabir2018NeuralApplications,Khosravi2011ComprehensiveAdvances} and a summary is provided below.

In forward uncertainty quantification, data uncertainty is estimated by propagating uncertain inputs through the network. Typical algorithms include Bayesian Neural Networks (BNN), quantile regression, Lower Upper Bound Estimation (LUBE), and mean-variance estimation. BNNs \cite{Blundell2015WeightNetworks} learn distributions over model weights rather than point estimates. A prior distribution is first imposed on the model parameters, and then Bayes rule $P(w|D) \propto P(w)P(D|W)$ is used to update the model parameters. While BNN can characterize the uncertainty with probability distributions, it is typically regarded as being too computationally expensive and having too strong distributional assumptions \cite{Pearce2018High-qualityApproach,Khosravi2011LowerIntervals}. To mitigate the problem of representing uncertainty in deep learning without sacrificing either computational complexity or test accuracy, dropout training in deep neural networks (NNs) is casted as approximate Bayesian inference \cite{Gal2016DropoutLearning}, and have since been used widely in various applications \cite{Li2020GraphPrediction,Ryu2019AQuantification,Sicking2020WassersteinDropout}. An alternative is to directly model the uncertainty of the dependent variable as an output node of the model. Quantile regression \cite{Koenker2001QuantileRegression} is one such model that directly outputs a particular quantile of the dependent variable instead of the mean. However, quantile regression is limited to estimating one quantile at a time and may face the issue of crossovers of modelled quantiles. To address these issues, LUBE \cite{Khosravi2011LowerIntervals, Pearce2018High-qualityApproach} directly outputs the specified prediction interval bounds. The bounds were formulated on the principle that the prediction intervals should cover the pre-specified amount of data points with the widths of the intervals as narrow as possible. A drawback of LUBE is that the LUBE loss function is difficult to minimize in complex networks; in past studies, only shallow networks are used. Despite computational issues, LUBE also suffers from the limitation that quantification is addressed as a mapping problem rather than a curve fitting problem and only one set of significance level can be estimated at once. To characterize the distribution of the predicted value, Mean Variance Estimation (MVE) \cite{Nix1994EstimatingDistribution} can be used. Instead of the often-used mean squared error loss for regression and cross entropy loss for classification, MVE minimizes the negative log likelihood (NLL) loss according to an assumed distribution of the dependent variable. MVE is easy to implement, but the caveat is that one single variance value may not do justice to asymmetric distributions, and that it assumes $\hat{y} \approx y$ when estimating $\hat{\sigma}$ and can lead to inaccurate prediction intervals when the model uncertainty is large\cite{Dybowski2009ConfidenceNetworks}. This asymmetric distribution is quite common in travel data, as the travel ridership is normally bounded above zero, thus violating the assumption of a symmetric distribution in the standard MVE. %However, as demonstrated in our experiments (Section \ref{model_vs_data_unc}), the suggested model architecture yields very small model uncertainty, and this assumption is therefore valid.

In inverse uncertainty quantification algorithms, model uncertainty is quantified by post-estimation model calibration. The most frequently used methods are bootstrapping and model ensembles \cite{Heskes1997PracticalIntervals,Lakshminarayanan2016SimpleEnsembles}. Since all of model specification, training sample, and model initialization affect model uncertainty, both methods involve training multiple neural networks, while varying one of the three factors that could contribute to model uncertainty and holding the other two constant. Bootstrapping refers to multiple trainings with re-sampled versions of the training set, accounting for the sampling bias, while holding model specification and model initializations the same. Model ensembling refers to multiple trainings with different parameter initializations, accounting for the parameter identification factor, while holding model specification and the training set the same. Uncertainty from model functional form limitations is generally not studied in deep learning models, since neural networks are overparameterized and regarded as universal approximators. 

\subsection{Uncertainty in Travel Demand}
While it is important to know the expected value, it is widely acknowledged that uncertainty compounds in multi-stage models\cite{Zhao2002TheAnalysis} and should also be considered in prediction\cite{Rasouli2012UncertaintyAgenda}. Without uncertainty considerations, the models typically assume homoskedasticity (constant variance). If violated, the assumption of homoskedasticity was shown to compromise the reliability of predicted point ridership of subway demand under the ARIMA-GARCH framework \cite{Ding2018UsingVolatility}. Research has been done on heteroskedastic variants on models including ARIMA-GARCH\cite{Chen2020SubwayData}, ARIMA-GRACH with adaptive Kalman filters\cite{Guo2014AdaptiveQuantification}, discrete choice models\cite{Petrik2016MeasuringModels}, and activity-based travel demand models\cite{Cools2010ASSESSMENTFEATHERS}. However, the discussion on uncertainty and heteroskedasticity in the deep learning framework is quite limited. One recent paper explored the quantification of heteroskedastic noise by training a CNN-LSTM model to fit not only the mean value but also the quantiles of the traffic demand distributions\cite{Rodrigues2020BeyondProblems}. Another discussed the quantification of model uncertainty through Monte-Carlo dropouts\cite{Li2020GraphPrediction}. 

\begin{comment}
In other fields of study, methods have been developed to model uncertainty in the deep learning framework. For example, researchers used deep learning to model the uncertainty in electricity load\cite{Quan2014UncertaintyForecasting}, survey responses\cite{Ding2020IncorporatingRegularization}, weather\cite{Wang2019DeepForecasting}, underwater depth\cite{Marques2020AEnvironment}. 
\end{comment}

Summary – A lot of recent efforts have been focused on variations of the algorithms mentioned above to adapt to different applications. In practice, forward and inverse algorithms are often coupled. There is no single algorithm that outperforms all others in all occasions. The choice of algorithms involves trade-offs among computational complexity, rigidity of assumptions, the desired coverage of prediction intervals, and characteristics of the dataset. 

\section{Problem Formulation}
Suppose we observe a transportation system over a period of time. Spatially, the system is divided into $S$ regions, indexed by $s=1,...,S$. Temporally, consider a total of $T$ time periods indexed by $t=1,...,T$. Let $y_{st}$ represent the demand in region $s$ in time period $t$, and $\mathcal{Y}_t \in \mathbb{R}^{S}$ the demand for all regions at time $t$. The goal of the prediction task is to forecast $\mathcal{Y}_{t}$ given information up to time $t-1$.

There are three types of covariates: time-specific ($\mathbf{X}^T$), region-specific ($\mathbf{X}^S$), and spatiotemporal ($\mathbf{X}^{ST}$). Time-specific covariates $\mathbf{X}^T$ are attributes that not location specific and vary only with time. Weather is one such example if the the system is defined to be within a relatively small spatial entity (such as a city). Region-specific covariates $\mathbf{X}^S$ are attributes that vary spatially and assumed to be constant for the considered time duration. For example, demographics are region-specific as far as short and medium term forecasts are considered. The last type is spatiotemporal, where the covariates $\mathbf{X}^{ST}$ vary both temporally and spatially. For example, scheduled service level is a spatiotemporal variable. Depending on data availability and relevance, the independent variables in a final prediction model for $\mathcal{Y}_{t}$ could contain one or more types of covariates that are denoted in general as $\mathbf{X_{t}}=\{ \mathbf{X}^T_t, \mathbf{X}^S, \mathbf{X}^{ST}_t \}$.

As previously mentioned, the goal is not only to predict $\mathcal{Y}_{t}$, but also the associated uncertainty measures. Here we resort to assuming a normal distribution for the demand estimates, where each $y_{st}$ follows a truncated normal distribution with mean $\hat{y_{st}}$ and variance $\hat{\sigma}^2_{st}$. Since demand must be non-negative, the distribution is left-truncated at $0$ to make the support of the distributions $\mathbb{R}_+$. Truncated Guassian distribution is used because it has stable performance and nice properties. For example, lognormal distributions are less stable when demand is close to 0; and Gaussians have nice expressions when models are ensembled. 

Further, it is assumed that the distributions of $y_{st}$ are independent from each other conditioned on the independent variables since the independent variables contain both spatial and temporal attributes, so that the total likelihood can be obtained by multiplying the likelihood of each $y_{st}$ for all $s$ and $t$ in scope.

\section{Methodology}

For this application, the prediction of public transit demands using deep learning is considered. A graph structure is assumed to account for spatial relationships. Temporally, the LSTM model is adopted due to its superior predictive performance. Since the primary interest lies in the prediction interval of short-term travel demand using methods compatible with deep learning and the prediction horizon is short, the algorithm needs to be easy to implement and not computationally inhibitive. Therefore, a TMVE-GCN in conjunction with model ensembles was formulated to investigate the uncertainty structure in spatiotemporal short-term travel demand. MVE requires a distribution of the dependent variable to be specified. To account for the nonnegativity of travel demand, a truncated normal distribution is proposed. The proposed algorithm can directly quantify uncertainty measures in a TMVE-GCN model, has the flexibility to fuse multi-source information, and can be optimized conveniently by back propagation. The proposed model can also be easily adapted to other systems with a graph structure; in spatial systems where grid is a better representation, graph convolutions can be substituted by standard grid convolutions. This section is structured as follows: addressing data uncertainty, addressing model uncertainty, model architecture accounting for spatial-temporal correlations, and model evaluation. 

\subsection{Data Uncertainty}

Mean variance estimation aims to capture data uncertainty $\sigma^2_{data}$ by characterizing the $\epsilon$ term in $y=f(x)+\epsilon$, and use maximum likelihood estimation (MLE) in model training to fit a distribution. Let $f(\cdot)$ represent the input-output mapping created by the TMVE-GCN neural network, $W$ represent the collection of model weights, the model can be written as:
\begin{equation}
    \begin{split}
        &\mathcal{Y}_{t} \sim \mathcal{N}(\hat{\mathcal{Y}}_{t}, \hat{\sigma}^2_{t})\\
        &\hat{\mathcal{Y}}_{t}, \hat{\sigma}^2_{t} = f_W(\mathbf{X_{t}})
    \end{split}
\end{equation}

where $\hat{\mathcal{Y}}_{t} = [\hat{y}_{st}, \forall s \in S], \hat{\sigma}^2_{t} = [\hat{\sigma}^2_{st}, \forall s \in S]$. Although the neural network produces a vector that contains information for all spatial units, the mean and variance for each spatial unit is assumed to be independent (conditioning on the input features), and the likelihood can be calculated separately and multiplied together. 

Owing to the non-negativity of the travel demand, the normal distribution is left truncated at 0 during model training. Regardless of the fitted distribution, the likelihood of observing negative demands is 0, so that the normalization constant of the density distribution is $1-\Phi(0)$ instead of 1. Let $\phi_{W}$ and $\Phi_{W}$ represent the  probability density function and the cumulative distribution function of the non-truncated normal distribution characterized by model weights $W$. The 
density of the truncated distribution $\tilde{\phi}_{W}(y)$ can be obtained by re-weighting the non-truncated density $\phi_{W}(y)$ by the probability that the demand is above 0 in the estimated distribution. 
\begin{equation}
    \tilde{\phi}_{W}(y) = \frac{\phi_{W}(y)}{1-\Phi_W(0)}, y \geq 0
\end{equation} 

Therefore, given the mean $\hat{y}_{st}$ and variance $\hat{\sigma}^2_{st}$ from the model weights $W$ and the input $\mathbf{X}_{t}$, the log likelihood of an observed demand $y_{st}$ for region $s$ during time period $t$ is:

\begin{equation}
    \begin{split}
        &\text{log } \tilde{\phi}_{W}(y_{st}|\hat{y}_{st}, \hat{\sigma}^2_{st}) \\
        &= \text{log } \frac{\phi_{W}(y_{st}|\hat{y}_{st}, \hat{\sigma}^2_{st})}{1-\Phi_{W}(0|\hat{y}_{st}, \hat{\sigma}^2_{st})} \\
        &= \text{log } \phi_{W}(y_{st}|\hat{y}_{st}, \hat{\sigma}^2_{st}) - \text{log } (1-\Phi_{W}(0|\hat{y}_{st}, \hat{\sigma}^2_{st})) 
    \end{split}
\end{equation}

MLE is equivalent to minimizing the negative log likelihood (NLL). A NLL loss function based on the joint density of all observations is formulated based on two assumptions. First, along the temporal dimension, the time series have a relatively short memory, implying that the observations become independent when the lookback periods are taken into account. Second, along the spatial dimension, the demand for each region $s$ during time period $t$ is conditionally independent given $X_t$. Combining the spatial and temporal independence assumptions, the loss function is simply the product of the probability density of all observations:

\begin{equation}
\begin{split}
    \text{NLL} &= -\sum_{s,t} \text{log } \tilde{\phi}_{W}(y_{st}|\mathbf{X_t}) \\
    &= -\sum_{s,t} \left[ \text{log } \phi_{W}(y_{st}|\mathbf{X_t}) - \text{log } (1-\Phi_{W}(0|\mathbf{X_t})) \right]\\
    &= \sum_{s,t} \frac{\text{log } (\hat{\sigma}_{st}^2)}{2} + \frac{(y_{st} - \hat{y}_{st})^2}{2\hat{\sigma}_{st}^2} \\
    &+\text{log } (1-\Phi_{W}(0|\mathbf{X_t})) + constant
\end{split}
\end{equation}


\subsection{Model Uncertainty}
To capture model uncertainty $\sigma^2_{model}$, we use the deep ensembles method proposed in \cite{Lakshminarayanan2016SimpleEnsembles}. Among the three sources of model uncertainty mentioned in Section \ref{uncertainty_framework}, the literature on uncertainty using deep learning generally ignores model mis-specification since neural networks are considered to have low bias and high variance. Model uncertainty coming from sampling is typically addressed by bootstrapping, where different training sets are formed by sampling the training data with replacement. Lastly, model uncertainty from model identification can be quantified by ensembling multiple independently trained models. However, past works have suggested that bootstrapping hurts performance \cite{Lakshminarayanan2016SimpleEnsembles, Lee2015WhyNetworks.} since a bootstrapped sample sees 63\%\footnote{The probability of an item being picked in a sample of size $N$ with replacement in $N$ experiments is $1-(1-1/N)^N$, which approximates to $1-e^{-1} \approx 0.63$ for a large $N$.} unique data points on average. In our experiments, we also observed that training on the entire training set with shuffling and random initializations of the neural networks yielded better performance than combining bootstrapping and ensembling. Therefore, bootstrapping was not used in estimating model uncertainty. The deep ensembles method used in the case study is described below.

The model is estimated $K$ times independently with different initial conditions. The ensemble prediction is treated as a uniformly-weighted mixture of the $K$ estimates and further approximated as a Gaussian distribution whose mean and variance are respectively the mean and variance of the mixture. Suppose $\mathcal{Y}_k, \sigma_k^2$ are the estimated mean and variance for estimate $k$. The ensembled mean $\mathcal{Y}_*$ and variance $\sigma_*^2$ are given by:

\begin{equation}
    \begin{split}
        &\mathcal{Y}_* = \frac{1}{K} \sum_k{\mathcal{Y}_k}\\
        &\sigma_*^2 = \frac{1}{K} \sum_k{(\sigma_k^2 + \mathcal{Y}_k^2)} - \mathcal{Y}_*^2 
    \end{split}
\end{equation}

\subsection{Model Architecture}
Figure \ref{fig:arch} shows the proposed architecture, consisting of four components: GCN-LSTM for \textbf{r}ecent observed demand, and spatiotemporal linear layer of last week's observation (\textbf{h}istory), \textbf{s}cheduled service (for transit systems only), and weather (tem\textbf{p}erature and \textbf{p}recipitation). The contribution of the four components are indexed by $r,h,s,p$, respectively, and summed to the final prediction:
\begin{equation}
\begin{split}
    \mathcal{Y} = \mathcal{Y}^r + \mathcal{Y}^h + \mathcal{Y}^s + \mathcal{Y}^p \\
    \sigma^2 = \sigma^2_r + \sigma^2_h + \sigma^2_s + \sigma^2_p
\end{split}
\end{equation}
Formulations of each of the four components are detailed in subsequent sections.
\begin{figure*}[ht]
    \centering
    \resizebox{0.75\linewidth}{!}{
    \includegraphics[width=\linewidth]{architecture.png}}
    \caption{Proposed model architecture. The model processes past demand information using LSTM and graph convolution, with the addition of auxiliary information such as weather and service schedule to produce mean and variance estimates simultaneously.}
    \label{fig:arch}
\end{figure*}

\subsubsection{Spatial Encoding by Multi-Graph Convolutions}
In order to produce the predictions $\hat{\mathcal{Y}}$ and $\hat{\sigma}^2$, spatiotemporal correlations with past demand is considered. In recent years, advances in graph neural networks have been made to account for spatial correlations beyond local grid convolutions in Convolution Neural Networks (CNN). The methods can be roughly divided into two categories: spectral methods that transform a signal with a filter to the Fourier domain, and non-spectral methods that operate directly in the graph domain. The spectral methods used to be prohibitively expensive due to the need to compute eigendecompositions. To circumvent this problem, Defferrard et al. proposed a fast localized spectral filter \cite{Defferrard2016ConvolutionalFiltering} and Kipf and Welling further simplified it with a first-order polynomial approximation \cite{Kipf2017Semi-supervisedNetworks}. The latter formulation has an elegant mathematical form and has gained popularity in a lot of graph applications. Here we adopt the convolution formulation proposed by Kipf and Welling. Suppose we have $L_g$ graph convolutional layers and the output of the hidden layers is denoted as $H^{(l)}$, $l=1,...,L_g$, we have the following layer-wise propagation rule:

\begin{equation}
    H^{(l+1)} = \sigma(\Tilde{D}^{-\frac{1}{2}}\Tilde{A}\Tilde{D}^{-\frac{1}{2}}H^{(l)}W^{(l)})
\end{equation}

where $\sigma(\cdot)$ is an activation function (most commonly ReLU); $\Tilde{D}_{ii}=\sum_j{\Tilde{A}_{ij}}$ is the degree matrix; $\Tilde{A} = A+I_N$ is the adjacency matrix with added self-connections; and $W^{(l)}$ is the trainable weights of layer $l$.

Graph convolution layers require upfront access to the global structure of the graph in the form of adjacency matrices $(A)$. Different types of spatial relationships can be defined through different adjacency matrices. Convolutional outputs from multiple adjacency matrices are summed to generate the final output. Suppose $R$ adjacency matrices, indexed by $r$, are defined for a graph, the multi-graph layer-wise propagation rule becomes 
\begin{equation}
    H^{(l+1)} = \sigma(\sum_{r=1}^R{\Tilde{D}_r^{-\frac{1}{2}}\Tilde{A}_r\Tilde{D}_r^{-\frac{1}{2}}H^{(l)}W_r^{(l)}})
\end{equation}

In this study, four types of adjacency matrices are considered: Euclidean distance $A_{E}$, network distance $A_{N}$, network connectivity $A_{C}$, and functional similarity $A_{F}$. 

Euclidean distance adjacency matrix is defined as
\begin{equation}
[A_{E}]_{ij} = \frac{1}{\text{Euclidean Distance}(i, j)}
\end{equation}
where Euclidean distance is defined as the straight-line distance between regions $i$ and $j$. 

Network distance adjacency matrix is defined as
\begin{equation}
[A_{N}]_{ij} = \frac{1}{\text{Network Distance}(i, j)}
\end{equation}
where network distance is defined as the distance between regions on the defined network. For example, with rail data, network distance is the distance between stations on the rail lines. With normal traffic, network distance can be taken as the travel time or driving distance. Both the Euclidean distance and network distance are meant to capture the pair-wise geographical relationships as shorter distance might signal similarities in ridership source, built environment, demographics, etc.

Network connectivity adjacency matrix is defined as
\begin{equation}
[A_{C}]_{ij} = \begin{cases}
1 & \text{if the two regions are adjacent}\\
0 & \text{otherwise}
\end{cases}
\end{equation}
In addition to being correlated by distance, this formulation gives a direct 0/1 formulation of adjacency that accounts for the local convolution in the immediate surroundings (similar to that of CNN).

Lastly, functional similarity adjacency matrix captures semantic relationships, encoded with demographic and built environment properties. Even though two regions might be distant from each other, their ridership demands could have similar patterns. For example, if both regions are of residential use with similar population and income, it is highly likely their peak ridership patterns are similar due to residents commuting. Let $F_i$ represent the vector of functionalities of the catchment area of region $i$. Catchment areas are areas of an arbitrary size centered at transit stations. It is assumed that people within the catchment area are potential passengers that feed into the transit station, in this case, based on the spacing of the transit system in Chicago, the area radius was set to 350 meters. Functionalities include population, jobs, percent low income, percent minority, percent adults, number of schools, shops, restaurants, etc. Functional similarity between two regions is defined as the distance between the normalized (where each measure is normalized to $\in [0,1]$, to eliminate the difference in the attribute magnitudes) region-specific property vectors. 

\begin{equation}
[A_{F}]_{ij} = \frac{1}{\sqrt{(F_i-F_j)^T(F_i-F_j)}}
\end{equation}

Different combinations of adjacency matrices were tested in our experiments. The sum of the four adjacency matrices consistently yielded near-optimal results, while single or pairs of adjacency matrices may perform well in certain runs but really poorly in others. Therefore, in the final version of the model the sum of the four adjacency matrices was included.

\subsubsection{Temporal Encoding by LSTM}
The most commonly used approach to learn the temporal features in travel demand is long-short term memory (LSTM) networks, which were shown to achieve superior predictive performance compared to other methods for temporal prediction. This structure is well-documented in a lot of papers \cite{Chen2020ForecastingNetworks, He2020GC-LSTM:Network,Zhao2020Short-TermSystems, Rodrigues2020BeyondProblems}, and will not be discussed in detail here. In short, to predict the demand during time period $t$ with prediction horizon of 1 time period, the LSTM layers take the spatially encoded tensors for $l$ time periods (from $t-l$ to $t-1$) as inputs, propagate them down the layers through a series of input, forget, cell state (memory), and output gates, to output a temporally encoded tensor for each of the $l$ time periods in scope (from $t-l+1$ to $t$). To make the prediction, the encoded output from the last time step is decoded by fully connected layers to get the contribution of recent demand on the predicted mean ($\hat{\mathcal{Y}}^r_t$) and standard deviation ($\hat{\sigma}^r_t$).

Due to the cyclic nature of transit demand, a good estimator of demand is the observed value for the same region and time in the previous week. Let $D_{t} \in \mathbb{R}^S$ represent the observed demand vector during the same time period last week, and $W^{h} \in \mathbb{R}^{2 \times S}$ represent the trainable spatial temporal weight for last week's demand. This history information assumes a linear relationship in the model with spatiotemporal coefficients. Since recent history is quoted as the deviation from last week's ridership, it contains information on how last week's demand should be related to the current prediction. The station-specific weights are obtained from the spatiotemporal encoding of recent history. The contribution of last week's demand on the final prediction is given by $[\hat{\mathcal{Y}}_t^h, \hat{\sigma}_t^h] = W^{h}_t(\mathbf{X_{st}}) D_{t}$.

\subsubsection{Additional Information}
In addition to recent demand history, various exogenous factors considered are: service level and weather. In transit systems, it is commonly acknowledged that service level is an important factor affecting demand \cite{Currie2008EffectiveEvidence,Brechan2017EffectTravel}. However, the level of influence is not reliably quantified due to the inability to experiment with service levels in large-scale transit systems for the purpose of observing demand change. Here we make the attempt to account for this factor by including the difference in scheduled trips compared to last week to account for the demand increase/decrease due to increased/decreased service. Under normal circumstances, this service difference is often small. However, for situations where the reference day/predicted day is a holiday, or when there is a service adjustment, the model is more capable to reflect the changes and make more accurate predictions. The way that service level enters the model is similar to that of last week's demand: $[\hat{\mathcal{Y}}_t^s, \hat{\sigma}_t^s] = W^{s}_t S_{t}$, where $S_t$ represent the difference in the number of scheduled trips during time period $t$ from last week.

Additionally, weather conditions could affect some spontaneous travel demand. Since mild weather fluctuations are expected, the impact of weather on transit ridership is more evident when the weather is more extreme. The model takes daily deviations from average of precipitation $P_T$ and temperature $T_E$, and multiply them with spatiotemporal weights $W^p, W^t \in \mathbb{R}^{2 \times T \times S}$ to get $[\hat{\mathcal{Y}}_t^p, \hat{\sigma}_t^p]$.

\subsection{Evaluation}
The total prediction uncertainty can be measured by the prediction intervals that combine data and model uncertainty with the ensembled variances. Prediction intervals are computed using the ensembled mean and variance similar to the classical way of constructing the confidence intervals in regression. Formally, with significance level $1-\alpha$, the lower bound of the prediction interval is given by $L = max(0,\mathcal{Y}_*- z_{\alpha/2} \sigma_*)$, and the upper bound of the prediction interval by $U = \mathcal{Y}_*+ z_{1-\alpha/2} \sigma_*$, where $z_{\alpha/2}$ is the standard score. 

To evaluate the mean estimation, three metrics are proposed: mean absolute error (MAE), mean squared error (MSE), and Theil's inequality coefficient $U$. MAE and MSE are standard metrics used in prediction accuracy evaluations. Theil's inequality coefficient $U \in [0,1]$ is a metric that measures the similarity in the predicted and target sequence of numbers, the smaller the better \cite{Ahlburg1984ForecastDecomposition}. 
\begin{equation}
    U = \frac{\sqrt{\frac{1}{N}\sum_{n=1}^{N}{(\hat{y}_n-y_n)^2}}}{\sqrt{\frac{1}{N}\sum_{n=1}^{N}{\hat{y}_n^2}+\sqrt{\frac{1}{N}\sum_{n=1}^{N}{y_n^2}}}}
\end{equation} 
To assess the different aspects of prediction accuracy, Theil's U can be further decomposed into bias $U^M$, variance $U^S$, and covariance $U^S$. The bias proportion $U^M$ examines the relationship between the means of the predicted and target sequences, $U^S$ considers the ability to match the variations in the sequences (different from the predicted variance $\sigma$, this metric measures the variation in the mean sequence formed by mean predictions of different regions and time periods), and $U^C$ captures the residual unsystematic element of the prediction errors. 
\begin{equation}
    \begin{split}
        U^M = \frac{(\bar{\hat{y}} - \bar{y})^2}{\frac{1}{N}\sum_{n=1}^{N}{(\hat{y}_n-y_n)^2}} \\
        U^S = \frac{(\bar{\hat{\sigma}} - \sigma)^2}{\frac{1}{N}\sum_{n=1}^{N}{(\hat{y}_n-y_n)^2}}\\
        U^C = \frac{2(1-\rho)\hat{\sigma}\sigma}{\frac{1}{N}\sum_{n=1}^{N}{(\hat{y}_n-y_n)^2}}
    \end{split} 
\end{equation}
where $\rho$ is the correlation coefficient between the predicted and actual sequence, $\sigma$ is the standard deviation of the actual sequence, and $\hat{\sigma}$ is the standard deviation of the predicted sequence. By construction, $U^M + U^S + U^C = 1$, with the preferred outcome for $U^M$ and $U^S$ to be as close to 0 as possible and for $U^C$ to be as close to 1 as possible.

The evaluation of the prediction intervals is less straightforward, since it involves a tradeoff between the the probability of coverage and prediction interval width, measured by the Prediction Interval Coverage Probability (PICP) and Mean Prediction Interval Width (MPIW), respectively \cite{Pearce2018High-qualityApproach, Khosravi2011LowerIntervals,Kabir2018NeuralApplications}. Formally,
\begin{equation}
    PICP = \frac{1}{n}{\sum_{i=1}^{n}{c_i}}
\end{equation}
where $c_i$ is the indicator variable of whether observation $i$ falls within the prediction interval bounded by $L_i$ and $U_i$:
$c_i= 1$ if $L_i \leq y_i \leq U_i$, $c_i = 0$ otherwise. 
\begin{equation}
    MPIW = \frac{1}{n}{\sum_{i=1}^{n}{(U_i - L_i)}}
\end{equation}

Intuitively, a high-quality prediction interval should be narrow while covering a large proportion of data points. However, wider MPIW naturally leads to larger PICP. Therefore, this tradeoff poses a challenge in model selection since it is difficult for one model dominate the others in both metrics.

\section{Case Study}
The proposed method was implemented in PyTorch and the source code is available at \url{https://github.mit.edu/qingyiw/uncertainty_quantification}. This section describes the setup of the case study that uses data from the Chicago Transit Authority (CTA) rail system, including the data sources, the data format, and the benchmark models.

\subsection{Data}
The task is to predict rail demand in the next time period using its own history, bus and TNC demand in the surrounding area, as well as other auxiliary information such as service level, demographics, etc. Data from CTA's rail network was used for this case study. Two time periods were considered: before COVID-19 (August 1, 2019 - Feb 29, 2020) and during COVID-19 (April 1, 2020 - Oct 31, 2020). Significant changes took place in March 2020 when confirmed COVID-19 cases were growing exponentially. For both the CTA and the passengers, March 2020 was a transient period, therefore it was excluded from this analysis. At the same time, COVID-19 gives the opportunity to test the generalizability of the model from pre- to during- COVID-19 condition.

Since overnight demand is low, demand between 6am and 11pm was considered. The temporal unit of analysis was taken to be 1 hour. The CTA network has 145 rail stations in total. However, most of the ridership is concentrated in downtown and therefore only the 18 downtown stations were considered (Figure \ref{fig:cta_dt}). If a station is served by multiple lines, demand for all lines was aggregated as all lines share the same fare gates.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\linewidth]{cta_rail_downtown.png}
    \caption{Study area of downtown Chicago with the subway stations highlighted.}
    \label{fig:cta_dt}
\end{figure}

The dataset was split into 3 subsets along the temporal dimension: train, validation, and test. The training set was used to train models, the validation set to select the models, and performance of the selected model(s) was then reported on the test set. For each time period, the following data was available:

\subsubsection{Rail, Bus and TNC}
Rail tap-ins come from the CTA's smart card system. Each tap-in is associated with a timestamp and location. In a multi-modal system, other travel modes in the region may serve as informative indicators to the changes and fluctuations of rail riderships. Bus data also comes from CTA's smart card system and is tagged to each bus stop and timestamp. TNC data comes from the City of Chicago's Open Data Portal\footnote{\url{https://data.cityofchicago.org/Transportation/Transportation-Network-Providers-Trips/m6dm-c72p}}; it is associated with 15-minute time periods and census tracts. To link bus and TNC ridership with rail spatially, a catchment area of 350m meters was created around each rail station, and demand from bus stops was intersected and aggregated within each station catchment area. TNC demand was scaled based on the overlap between the catchment areas and census tracts. Visualization of average daily ridership is shown in Figure \ref{fig:data_viz}. The two time periods exhibit significant differences in demand patterns. Before COVID-19 the demand magnitude was stable, with a sharp drop observed around holiday times. During COVID-19, after the initial drop in March, a slow recovery can be observed starting April, especially for TNC. Between April and June of 2020, rear-door boarding policy was active, therefore no bus ridership was observed. 

\begin{figure}
    \centering
    \subfloat[]{\includegraphics[width=\linewidth]{before_demand_viz.png}}\\
    \subfloat[]{\includegraphics[width=\linewidth]{after_demand_viz.png}}
    \caption{Average Daily Ridership (a) Before COVID-19 and (b) During COVID-19}
    \label{fig:data_viz}
\end{figure}

\subsubsection{Service Level}
Service level, in the form of number of scheduled rail departures at each station for each hour, is obtained from General Transit Feed Specification (GTFS)\footnote{\url{https://transitfeeds.com/p/chicago-transit-authority/165}}.

\subsubsection{Demographics and POI}
Spatial attributes used to construct the functional similarity adjacency matrix include demographics and point of interest (POI). Since they are spatial only and do not vary with time, spatial attributes enter the graph convolution, but are not included in the explanatory variables. Demographics are obtained from the American Community Survey (ACS)\footnote{\url{https://www.census.gov/programs-surveys/acs/data.html}} and POIs from Open Street Map (OSM)\footnote{\url{https://planet.openstreetmap.org/}}. ACS data include total population, percent adults (25-50yrs), percent elders (65yrs+), percent white, number of jobs, percent commuters on public transit, average travel time to work, income per capita. POI data is a layer of points that include the number of entertainment venues, restaurants, schools, and shops, and is aggregated to the catchment area of each rail station. Demographics are quoted for each census tracts and a weighted average is calculated for the catchment area of each rail station. 

\subsubsection{Weather}
Precipitation and temperature can be downloaded from the National Centers of Environmental Information\footnote{\url{https://www.ncdc.noaa.gov/cdo-web/}} and the data resolution is daily.

\subsection{Models}
Two benchmark models were constructed:
\subsubsection{Last Week}
Taking $\mathcal{Y}^{h}_t$ as the predicted value, and going back 8 weeks to get the empirical standard deviations as the variance measure.

\subsubsection{Weighted Least Squares (WLS) Regression}
\begin{equation}
    \begin{split}
        \mathcal{Y}_t = \mathbf{X}_{t}\beta^{m} + \mathcal{Y}^{h}_t \lambda + \epsilon_t\\
        \epsilon_t \sim \mathcal{N}(0, \sigma_t), \sigma_t = \mathbf{X}_{t}\beta^{s}
    \end{split}
\end{equation}

where $\beta^m$ and $\beta^s$ are coefficients of the explanatory variables for the mean and variance, respectively; and $\lambda$ is the coefficient for $y$'s own history.

And three variations of the TMVE-GCN were constructed:
\subsubsection{TMVE-GCN}
The proposed model. Lookback periods considered were 2, 4, and 6. The neural network hyperparameter search space is presented in Table \ref{tab:hyperparameters}. A grid search in this space was done to find the optimal hyperparameter set.

\begin{table}[ht]
    \centering
    \caption{Hyperparameters}
    \begin{tabular}{l|c}
        \toprule
        Hyperparameter & Search Space \\
        \midrule
        \# GCN layers & 1, 2, 3 \\
        \# Units in hidden layers & 32, 64, 128, 256\\
        \# LSTM layers & 1, 2, 3 \\
        Dropout & 0.25, 0.5 \\
        Weight decay & 0.005, 0.01, 0.05 \\
        \bottomrule
    \end{tabular}
    \label{tab:hyperparameters}
\end{table}

\subsubsection{TMVE-GCN Ensemble}
Top five models on the validation set were selected to form the ensemble model. 

\subsubsection{TMVE-GCN-Homo}
The homoskedastic variation of TMVE-GCN. Instead of having the variance dependent on the spatiotemporal input values $\hat{\sigma}_{st}$, the variances of all observations are of the same value $\hat{\sigma}$ and optimized by negative log-likelihood loss.

\subsection{Evaluation}
Since the parameters of a truncated normal distribution are estimated, prediction intervals of arbitrary widths can be constructed. Throughout this work, we use the $95\%$ significance level ($z_{\alpha/2} = 1.96$) for evaluation. The models are evaluated both on the point prediction and the quality of the prediction interval. The metrics used and their categorizations are shown in Table \ref{tab:metrics}.

\begin{table}[]
    \centering
    \caption{Evaluation Metrics}
    \begin{tabular}{c|c|c}
        Metric & Prediction Interval & Point Prediction \\
        \toprule
        LogLikelihood & \checkmark & \checkmark \\
        MPIW & \checkmark & \\
        PICP & \checkmark & \\
        MAE & & \checkmark \\
        RMSE & & \checkmark \\ 
        Theil's U & & \checkmark \\ 
        \bottomrule
    \end{tabular}
    \label{tab:metrics}
\end{table}

\section{Results and Discussion}
This section presents and discusses the model results. First, we present different evaluation metrics to show that the proposed model achieves superior performance over the benchmark models. Then different uncertainty patterns are investigated to demonstrate the existence and importance of heteorskedasticity in the dataset. Lastly, model generalizability is shown by applying models trained with the pre-COVID data to the post-COVID test set.

\subsection{Model Performance}
Overall model performance is tabulated in Table \ref{tab:model_perf}. Three different types of metrics are used to evaluate the models. First, the composite NLL loss is used to train the network in order to precisely predict both the mean and variance. Second, PICP and MPIW evaluate the quality of prediction intervals. Third, MAE, RMSE, and Theil's U evaluate the quality of point estimates. Due to COVID-19, ridership dropped around 80\% and ridership patterns are very different (Figure \ref{fig:data_viz}) between the pre- and post-COVID periods. TMVE-GCN achieves better performance than the benchmark models in both time periods on the majority of the metrics.

% nll loss
\subsubsection{Composite Measures}

The composite NLL loss is used to train the network in order to achieve both objectives. Ideally, a good composite measure should be strongly positively related to measures for both purposes. Figure \ref{fig:nll_as_loss} shows the relationship betweeen NLL and Theil's U and MPIW for different model trainings. Only model trainings that achieve the intended 95\% PICP are considered. A generally positive correlation can be observed for both NLL vs. Theil's U and NLL vs. MPIW (although the relationship is very noisy in the during COVID-19 set), indicating the NLL is a good composite loss function to capture both the mean and variance of the predicted quantity. 

\begin{figure*}[ht]
    \centering
    \subfloat[]{\includegraphics[width=0.45\linewidth]{before_nll_u_mpiw_tradeoff.png}}
    \subfloat[]{\includegraphics[width=0.45\linewidth]{after_nll_u_mpiw_tradeoff.png}}
    \caption{NLL to measure both mean and PI quality (a) Before COVID-19 and (b) During COVID-19}
    \label{fig:nll_as_loss}
\end{figure*}

The TMVE-GCN models are able to achieve a significant improvement in log likelihood compared to the benchmark models. Since the log likelihood metric jointly evaluates the mean and variance, the higher log likelihood suggests that the TMVE-GCN model fits for predicting uncertainty without sacrificing the quality of average ridership prediction. We differentiate between the quality of mean and variance prediction in the following sections. % since the objective of the proposed models is to minimize negative log likelihood, while last week's model does not have an objective, and weighted least squares is designed to minimize RMSE. 

% uncertainty
\subsubsection{Quality of Uncertainty Estimates}

PICP and MPIW are used in conjunction to evaluate the quality of uncertainty prediction. In general, a positive correlation can be expected between PICP and MPIW. Namely, a wider interval is needed to cover more observations. Figure \ref{fig:model_perf_pi_quality} describes the tradeoff between the PI quality measures, MPIW and PICP. The metrics plotted are the average value across the test set, and each marker marks one instance of model training (with different hyperparameters). Marker shapes indicate model type, and marker colors indicate the dataset. Because COVID-19 caused a significant reduction in demand, the scale of the two datasets is of different magnitude, and therefore plotted on different y-axis scales. The increase is steep in Figure \ref{fig:model_perf_pi_quality} as PICP 0.95 is in the tail region of a normal distribution. In both analysis periods, PI widths achieving close to 100\% coverage were almost three times the ones for 95\%. While producing intervals that are short of the intended coverage would cause the decision-maker to be too optimistic about the demand variations, having wider than necessary interval widths results in decisions that are too conservative.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{picp_mpiw_tradeoff.png}
    \caption{Model Performance: Prediction Interval Quality}
    \label{fig:model_perf_pi_quality}
\end{figure}

% With the intended level being 95\%, the proposed model has coverages concentrated between 93\% and 99\%, whereas WLS yields coverages between 60\% and 70\%. Even though the interval widths from WLS are smaller, their coverage probabilities are too far from the intended level of 95\%. The other benchmark model - last week and empirical variance - achieves coverages around 90\%. However, with the the same interval widths, the proposed model achieves much higher PICPs. Therefore, the TMVE-GCN model dominates the benchmark models with respect to the uncertainty estimates. 

The prediction intervals constructed from the TMVE-GCN models successfully incorporate the true observations in the test set for around 95\% of the time with a reasonably narrow interval width. Although the interval widths from the two benchmark models are narrower than the TMVE-GCN model, both benchmark models do not cover the designated proportion (95\%) of points. Weighted least squares have the narrowest prediction interval but the coverage is significantly smaller than 95\% (60\% and 74\% for before and during COVID-19, respectively). The empirical uncertainty estimates cover around 90\% of the observations for both periods, but compared to the TMVE-GCN model, the interval is wider while covering fewer points.

The homoskedastic version of TMVE-GCN is very sensitive to the initial value of the variance and thus presents a trade-off in performance. The width and coverage of the prediction interval largely depend on the magnitude of the variance. The smaller the variance is initialized to, the narrower the resulting prediction interval width with less coverage probability. 
% On the other hand, smaller initial variance results in more accurate mean estimation but worse likelihood; a larger initial variance value results in better likelihood but worse mean estimation. This is due to the variance being represented by one parameter and mean is calculated from a huge neural network. Thus the appropriate learning rates are different. Using the same learning rate appropriate for the large network causes the variance parameter to converge too slowly, but using a larger learning rate will cause the rest of the network to break down. 
Since selecting the appropriate homoskedastic variance is out-of-scope, we present the trade-off by initializing the variance value to one and the average of empirical variance. In the table, the models are labelled TMVE-GCN-Homo-1 and TMVE-GCN-Homo-EV, respectively. TMVE-GCN-Homo-1 achieves the best mean prediction among all models, but really bad prediction intervals; whereas TMVE-GCN-Homo-EV produces the worst mean prediction but has comparatively better likelihood. However, the TMVE-GCN-Homo-EV's likelihood and prediction intervals are still worse than TMVE-GCN, demonstrating that travel demand is heteroskedastic and joint training achieves more balanced results.

% ensemble
Model uncertainty is not significant compared to data uncertainty, evidenced by the top training instances producing similar results. More will be discussed on the decomposition of data and model uncertainty in the next section.

% mean
\subsubsection{Point Estimate}
While obtaining more accurate uncertainty estimates, TMVE-GCN models did not sacrifice mean performance. The TMVE-GCN models achieve smaller MAE than the benchmark models. Since WLS is trained on minimizing RMSE, it achieves the best results on this metric, as well as better Theil's U estimates. But the decomposition shows that there is almost no bias $U^M$ in all models, most prediction errors lie in the unsystematic variations $U^C$, while the variation in the mean prediction $U^S$ is easier to capture during COVID-19 than before COVID-19. At first sight this is quite unexpected. But during COVID-19 people who are still on transit are mostly conducting essential trips, making the demand more predictable.

%
In summary, the TMVE-GCN models achieve overall good performance on both mean and uncertainty metrics. Only on the metrics that the models are specifically trained for (i.e. WLS uses RMSE), the TMVE-GCN models slightly underperform.


\begin{table*}[ht]
    \centering
    \caption{Model Performance}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
        & Composite & \multicolumn{2}{c|}{Prediction Interval} & \multicolumn{4}{c}{Point Estimate}\\
        \midrule
        Model & Negative LogLikelihood & MPIW (\#Tap-ins) & PICP & MAE (\#Tap-ins) & RMSE (\#Tap-ins)& Theil's U & Decomposition ($U^M/U^S/U^C$) \\
        \midrule
        \multicolumn{8}{c}{Before COVID-19 (Aug 2019 - Feb 2020)}\\
        \midrule
        Last Week & 100.4 & 517.5 & 0.8994 & 71.82 & 281.0 & 0.09611 & 0.01307 / 0.09997 / 0.887\\
        Weighted Least Squares & 142.2 & 238.9 & 0.7356 & 77.94 & 212.0 & 0.07232 & 0.02113 / 0.1466 / 0.8323\\
        GCN MVE Homo EV & 122.7 & 1.138e+03 & 0.9883 & 157.3 & 316.9 & 0.1095 & 0.1942 / 0.05481 / 0.751\\
        GCN MVE Homo 1 & 2.862e+04 & 14.37 & 0.206 & \bf{63.07} & \bf{206.8} & \bf{0.07042} & 0.004034 / 0.1598 / 0.8361\\
        GCN MVE & 94.38 & \bf{356.2} & \bf{0.9524} & 67.57 & 252.4 & 0.08659 & 0.01044 / 0.1598 / 0.8298\\
        GCN MVE Ensemble & \bf{94.1} & 397.1 & 0.9622 & 66.79 & 250.8 & 0.08596 & 0.0098 / 0.1554 / 0.8348\\
        \midrule
        \multicolumn{8}{c}{During COVID-19 (April 2020 - Oct 2020)}\\
        \midrule
        Last Week & 75.09 & 109.3 & 0.9241 & \bf{13.35} & 24.31 & 0.07027 & 0.007315 / 0.02735 / 0.9653\\
        Weighted Least Squares & 115.7 & 48.6 & 0.5943 & 13.77 & \bf{22.59} & \bf{0.06598} & 0.001239 / 0.00062 / 0.9981\\
        GCN MVE Homo EV & 80.22 & 85.81 & 0.9654 & 19.08 & 28.09 & 0.08379 & 0.1757 / 0.000251 / 0.824\\
        GCN MVE Homo 1 & 344.3 & 17.89 & 0.599 & 13.7 & 26.78 & 0.07906 & 0.000271 / 0.01142 / 0.9883\\
        GCN MVE & 70.7 & \bf{84.7} & \bf{0.9559} & 13.97 & 28.53 & 0.08346 & 0.002327 / 0.000162 / 0.9975\\
        GCN MVE Ensemble & \bf{70.44} & 80.89 & 0.9616 & 13.46 & 25.58 & 0.07543 & 0.0004447 / 0.01425 / 0.9853\\    
        \bottomrule
    \end{tabular}
    }
    \label{tab:model_perf}
\end{table*}

\subsection{Uncertainty Patterns}

\subsubsection{Prediction Interval Visualization}
The first row of Figure \ref{fig:pi} (abcd) visualizes the true demand, individual PIs, and ensembled PIs at the station with the largest observed demand (before: Clark/Lake, during: State/Lake), and the station with the lowest observed demand (before: Lasalle, during: Lasalle/Van Buren) for a day in the test set. The figures demonstrate the existence of significant heteroskedascity since the width of prediction intervals varies with time. High-demand stations appear to have narrower prediction intervals, compared to low demand stations, whereas the widths for low demand stations appear wider. However, in absolute terms, PI for high-demand stations are on average wider. Higher demand stations have larger absolute uncertainty but smaller relative uncertainty, which will be further investigated in the next section.

Figure \ref{fig:pi} enables a visual comparison of the PI quality across the models for different times of the day. During the peak hours, the benchmark models (blue and coral) often have intervals wider than the TMVE-GCN models, while the TMVE-GCN models already achieve the intended prediction interval coverage. At times when the benchmark models' interval widths are narrower, the narrower intervals sometimes fail to capture the true demand. During off-peak times, the differences are not significant. 

\begin{figure*}[ht]
    \centering
    \captionsetup[subfigure]{justification=justified,singlelinecheck=false}

    \resizebox{\linewidth}{!}{
    \subfloat[Before, Max flow]{\includegraphics[width=0.215\linewidth]{before_ens_pi_max_temp.png}}
    \subfloat[Before, Min flow]{\includegraphics[width=0.2\linewidth]{before_ens_pi_min_temp.png}}
    \subfloat[After, Max flow]{\includegraphics[width=0.2\linewidth]{after_ens_pi_max_temp.png}}
    \subfloat[After, Min flow]{\includegraphics[width=0.375\linewidth]{after_ens_pi_min_temp.png}}}
    \resizebox{\linewidth}{!}{
    \subfloat[Before, Max flow]{\includegraphics[width=0.215\linewidth]{before_model_data_unc_max.png}}
    \subfloat[Before, Min flow]{\includegraphics[width=0.2\linewidth]{before_model_data_unc_min.png}}
    \subfloat[After, Max flow]{\includegraphics[width=0.2\linewidth]{after_model_data_unc_max.png}}
    \subfloat[After, Min flow]{\includegraphics[width=0.395\linewidth]{after_model_data_unc_min.png}}
    }
    \caption{(a)(b)(c)(d): Prediction intervals; (e)(f)(g)(h): Data uncertainty vs. model uncertainty of max and min flow stations before and after COVID-19.}
    \label{fig:pi}
\end{figure*}

% \begin{figure*}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \includegraphics{combined_fig.png}}
%     \caption{Prediction intervals and data vs. model uncertainty of (a) Station with max flow before COVID-19, (b) Station with min flow before COVID-19, (c) Station with max flow during COVID-19, and (d) Station with min flow during COVID-19}
%     \label{fig:pi_unc}
% \end{figure*}

\subsubsection{Data Uncertainty vs. Model Uncertainty}\label{model_vs_data_unc}

Figure \ref{fig:pi}(efgh) demonstrates that prediction uncertainty mainly arises from the data but not the model uncertainty. Model uncertainty refers to the different results obtained from the same training set and model architecture, as shown by the variation of different predictions (grey intervals) in Figure \ref{fig:pi}. Although different initializations converge to the neural networks' different local minima, the demand forecast is quite stable in different model trainings. For both stations, model uncertainty is quite minor as the predicted demand are very close to each other compared to the estimated data uncertainty (green intervals from the ensembled TMVE-GCN model). Low model uncertainty suggests that there is little room for improvement in terms of reducing the uncertainty with the current set of explanatory variables. Therefore, the modelling focus should be the irreducible data uncertainty.

% \begin{figure}[ht]
%     \centering
%     \subfloat[]{\includegraphics[width=\linewidth]{before_model_data_unc_max.png}}\\
%     \subfloat[]{\includegraphics[width=\linewidth]{before_model_data_unc_min.png}}\\
%     \subfloat[]{\includegraphics[width=\linewidth]{after_model_data_unc_max.png}}\\
%     \subfloat[]{\includegraphics[width=\linewidth]{after_model_data_unc_min.png}}\\
%     \caption{Data Uncertainty vs. Model Uncertainty of (a) Station with max flow before COVID-19, (b) Station with min flow before COVID-19, (c) Station with max flow during COVID-19, and (d) Station with min flow during COVID-19}
%     \label{fig:data_model_unc}
% \end{figure}

\subsubsection{Absolute Uncertainty vs. Relative Uncertainty}

\begin{figure*}[ht]
    \centering
    \subfloat[]{\includegraphics[width=0.45\linewidth]{before_flow_vs_mpiw.png}}
    \subfloat[]{\includegraphics[width=0.45\linewidth]{after_flow_vs_mpiw.png}}
    \caption{Demand vs. Uncertainty (a) Before COVID-19 and (b) During COVID-19}
    \label{fig:unc_vs_flow}
\end{figure*}

Figure \ref{fig:unc_vs_flow} further investigates the relationship between MPIW and average travel demand at all stations for the ensembled model. The results can be used to examine the hypothesis that prediction intervals are correlated with the magnitude of observed travel demand. For both periods, there is a strongly positive relationship between MPIW and average travel demand, shown by the blue points, and a strongly negative relationship between MPIW normalized by demand and average travel demand, shown by the red points. Stations with higher demand have higher absolute uncertainty and smaller relative uncertainty. In practice, this proportional relationship informs the decision maker to build in  capacity buffers relative to average flow for each station instead of buffers of absolute sizes.

\subsection{Model Generalizability}

Within each dataset, the validation and test sets are days immediately following the training set, leaving unanswered the generalizability question particularly for the significant disruptions introduced by the COVID. In this section, we will demonstrate that the model performance is still of high-quality after a longer period of time without adding new data to the training set, by applying the models trained with before COVID-19 demand to the during COVID-19 test set. Figure \ref{fig:ro_test} shows the mean and prediction interval for the max and min demand stations, respectively. Three models are compared, the first one is the ensemble model trained with the during COVID-19 demand data (April - Oct, 2020), serving as the benchmark model. The other models are the best performing and ensemble model trained on before COVID-19 demand data (Aug 2019 - Feb 2020). 

% \begin{figure*}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \centering
%     \includegraphics{rotest_combined.png}}
%     \caption{Model Transfer Performance (a) Mean prediction (station with max flow), (b) Mean prediction (station with min flow), (c) PI (station with max flow), and (d) PI (station with max flow)}
%     \label{fig:ro_test}
% \end{figure*}

\begin{figure*}[ht]
    \centering
    \resizebox{\linewidth}{!}{
    \subfloat[]{\includegraphics[width=0.215\linewidth]{rotest_max_mean.png}}
    \subfloat[]{\includegraphics[width=0.19\linewidth]{rotest_min_mean.png}}
    \subfloat[]{\includegraphics[width=0.21\linewidth]{rotest_max_pi.png}}
    \subfloat[]{\includegraphics[width=0.45\linewidth]{rotest_min_pi.png}}}
    \caption{Model Transfer Performance (a) Mean prediction (station with max flow), (b) Mean prediction (station with min flow), (c) PI (station with max flow), and (d) PI (station with max flow)}
    \label{fig:ro_test}
\end{figure*}

Since the model inputs are demand from the previous week and demand differences hours before to the same time period in the previous week, as long as the week-to-week variation is not drastic, the model should be able to adjust to new time periods reasonably well without additional training. Figure \ref{fig:ro_test}a and \ref{fig:ro_test}b demonstrate that the mean prediction is not very different from model to model; while Figure \ref{fig:ro_test}c and \ref{fig:ro_test}d show that the the uncertainty bounds become looser if the models are directly applied without re-training. 

Table \ref{tab:model_robust_test} quantifies this performance difference. There is a 3-4\% decrease in performance in log likelihood, MAE, and Theil's U. The decomposition shows a slight increase in bias because of the transfer. Regarding the uncertainty measures, the interval widened by 14 and 11.5 passengers, while the coverage increased by 2.8\% and 2.3\%. Under the same training and testing set, a width increase would also be expected from coverage increase. To estimate that effect, a linear best fit line was constructed from the points in Figure \ref{fig:model_perf_pi_quality}. Interpolating from the best fit line, a 13.7 and 11.3 width increase can be expected for the same percentage increase in coverage. Although model transfer made the model more conservative and the coverage is higher than the intended 95\%, the decrease in performance was within the range of the models trained on same period data. As a comparison, the generalizability of WLS is also presented (using last week's reference is not included since it does not involve estimated parameters). The transferred WLS model is significantly worse than the proposed model in all evaluation metrics.

\begin{table*}[ht]
    \centering
    \caption{Model Generalizability Test}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
        \toprule
        Train Set & Test Set & Model & Negative LogLikelihood & MPIW & PICP & MAE & RMSE & Theil's U & Decomposition ($U^M/U^S/U^C$) \\
        \midrule
        During & During & Ensemble & 70.44 & 80.89 & 0.9616 & 13.46 & 25.58 & 0.07543 & 0.0004447 / 0.01425 / 0.9853\\
        Before & During & Ensemble & 72.65 & 94.99 & 0.9895 & 14.12 & 25.57 & 0.07401 & 0.03663 / 0.004673 / 0.9587\\
        Before & During & Single & 72.21 & 92.49 & 0.9848 & 14.04 & 25.41 & 0.07377 & 0.02297 / 0.002118 / 0.9749\\
        Before & During & WLS & n/a & 120.8 & 0.873 & 34.85 & 54.87 & 0.1526 & 0.044 / 0.06648 / 0.8895\\
        \bottomrule
    \end{tabular}
    }
    \label{tab:model_robust_test}
\end{table*}

\section{Conclusion}
This paper is motivated by the observation that the predominant research focuses on using deep learning for only the estimation of the mean travel demand but not its uncertainty. To fill this gap, we designed the TMVE method for a Graph Convolutional LSTM model to quantify the spatiotemporal uncertainty in travel demand. This joint TMVE approach was then applied to rail demand in Chicago, yielding the following major findings. 

First, significant travel demand uncertainty does exist. It was fully demonstrated by the higher performance of the heterogeneous TMVE-GCN model than the homogeneous one. It was further articulated by the trade-off between the PICP and MPIW metrics. Although a strict dominance regarding uncertainty quantification is challenging due to the trade-off, our results illustrate how and why the TMVE-GCN model can effectively quantify demand uncertainty, successfully achieving the targeting interval width and coverage probability. Second, the pattern of the spatiotemporal uncertainty can be revealed by the TMVE-GCN algorithm. The uncertainty prediction produced by the TMVE-GCN method is more accurate than the benchmark models. The degree of uncertainty (variance) is highly correlated with the magnitude of the travel demand (mean). This finding is consistent with the statistical intuition that the sum of a larger number of random variables tends to have a larger variance. Third, we showed that the model training is stable. Model uncertainty is relatively small as opposed to data uncertainty, suggesting that more attention should be paid towards capturing the exact structure of the error term. Lastly, the models can transfer to future time periods reasonably well without re-training. Overall, this work is one of the first that demonstrates travel demand uncertainty through the deep learning framework, applies the novel TMVE-GCN algorithm to a major US metropolitan area using high-granular travel demand data, and articulates the spatiotemporal uncertainty structure.

This TMVE algorithm is a computationally efficient approach, but many other methods can be applied. For example, the deep Bayesian neural networks can provide a full probability distribution with spatiotemporal structure captured. Another approach of estimating the lower and upper bound (LUBE) has less rigid probability assumption and directly targets the two bounds of the prediction intervals. These methods always involve a trade-off between stringent assumptions and computational efficiency, so a definitive choice is hard to make. Nonetheless, future studies should investigate the alternative methods to corroborate with our findings. From a practical perspective, a remaining question is how to take full advantage of the learnt travel demand uncertainty to inform the design of transport system and policies. Travel demand uncertainty is the source of many transport problems. For example, a surge in travel demand in automobile usage could cause the congestion that starts in a region and propagates into the whole urban road network. A sudden plummet in travel demand, such as that caused by COVID-19, can lead to the depletion of many transport industries' revenue and the bankruptcy of many mobility companies. A better understanding of the uncertainty structure in travel demand provides the opportunities for engineers and policy makers to take preemptive strategies before disruptions happen. This work shall naturally lead to further robust system and policy design in transport, which we unfortunately cannot address in this study, but has to leave to the future.



% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.





\begin{table*}[ht!]
    \centering
    \caption{Model Performance (Graph Convolutional Networks)}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c}
        \toprule
        & \multicolumn{1}{c|}{Composite Metric} & \multicolumn{3}{c|}{Uncertainty Estimate Metrics} & \multicolumn{2}{c}{Point Estimate Metric}\\
        \midrule
        Model & Negative LogLikelihood & Calibration Error & MPIW (\#Tap-ins) & PICP & MAE (\#Tap-ins) & MAPE\\
        \midrule
        \multicolumn{6}{c}{Pre COVID}\\
        \midrule
        HomoG-GCN (deterministic) & 114.1 & 0.123  & 386.9 & 95.7\% & \textbf{53.47} & \textbf{8.42\%} \\
        Pois-GCN & 183.8 & 0.118 & 63.08 & 61.1\% & 61.02 & 9.60\%\\
        HetG-GCN & 94.76 & 0.046 & \textbf{363.1} & \textbf{95.0\%} & 64.54 & 10.2\%\\
        TG-GCN & 94.39 & 0.048 & 381.0 & 95.6\% & 66.95 & 10.5\%\\
        Lap-GCN & \textbf{92.69} & \textbf{0.010} & 393.5 & 96.8\% & 66.22 & 10.4\% \\
        GEns-GCN & 94.11 & 0.034 & 397.0 & 96.2\% & 66.40 & 10.5\% \\
        \midrule
        \multicolumn{6}{c}{Post COVID}\\
        \midrule
        HomoG-GCN (deterministic) & 84.16 & 0.101 & 88.45 & 95.9\% & 13.72 & 15.4\%\\
        Pois-GCN & 89.24 & 0.089 & 28.40 & 74.1\% & 13.63 & 15.3\%\\
        HetG-GCN & 71.03 & \textbf{0.018} & \textbf{71.03} & \textbf{95.4\%} & 13.61 & 15.3\%\\
        TG-GCN & 70.86 & 0.024 & 73.51 & 96.0\% & \textbf{13.41} & \textbf{15.1\%}\\
        Lap-GCN & 71.32 & 0.025 & 77.27 & 97.0\% & 13.71 & 15.4\%\\
        GEns-GCN & \textbf{70.83} & 0.026 & 73.04 & 95.8\% & 13.50 & 15.2\% \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:model_perf_gcn}
\end{table*}

\begin{table*}[ht!]
    \centering
    \caption{Model Performance (Graph Attention Networks)}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c|c}
        \toprule
        & \multicolumn{1}{c|}{Composite Metric} & \multicolumn{3}{c|}{ Uncertainty Estimate Metrics} & \multicolumn{2}{c}{Point Estimate Metric}\\
        \midrule
        Model & Negative LogLikelihood & Calibration Error & MPIW (\#Tap-ins) & PICP & MAE (\#Tap-ins) & MAPE\\
        \midrule
        \multicolumn{7}{c}{Pre COVID}\\
        \midrule
        HomoG-GAT (deterministic) & 131.8 & 0.119 & 385.7 & 94.9\% & 64.50 & 10.2\%\\
        Pois-GAT & 190.3 & 0.125 & 65.61 & 60.0\% & \textbf{62.36} & \textbf{9.81\%} \\
        HetG-GAT & 94.79 & 0.037 & \textbf{383.4} & \textbf{94.9\%} & 67.49 & 10.6\% \\
        TG-GAT & 93.77 & 0.052 & 495.8 & 97.7\% & 68.42 & 10.8\% \\
        Lap-GAT & \textbf{92.72} & \textbf{0.019} & 383.9 & 96.5\% & 67.52 & 10.6\% \\
        GEns-GAT & 93.46 & 0.043 & 440.6 & 97.0\% & 66.26 & 10.4\% \\
        \midrule
        \multicolumn{7}{c}{Post COVID}\\
        \midrule
        HomoG-GAT (deterministic) & 82.77 & 0.101 & 88.63 & 96.5\% & \textbf{13.17} & \textbf{14.8\%} \\
        Pois-GAT & 90.59 & 0.084 & 28.01 & 73.4\% & 13.99 & 15.7\%\\
        HetG-GAT & 71.09 & \textbf{0.015} & \textbf{71.19} & \textbf{95.4\%} & 13.57 & 15.3\%\\
        TG-GAT & 71.18 & 0.021 & 73.03 & 96.0\% & 13.98 & 15.7\%\\
        Lap-GAT & 71.29 & 0.023 & 83.38 & 97.3\% & 13.53 & 15.2\% \\
        GEns-GAT & \textbf{70.83} & 0.026 & 73.04 & 95.8\% & 13.55 & 15.2\% \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:model_perf_gat}
\end{table*}


\begin{table*}[ht!]
    \centering
    \caption{Model Performance on TNC Data}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{p{2cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}}
        \toprule
        & Comp & \multicolumn{3}{c|}{Uncertainty Estimate} & \multicolumn{2}{c}{Point Estimate} \\
        \midrule
        Model & NLL & Cal. Err & MPIW & PICP & MAE & MAPE \\
        \midrule
        \multicolumn{7}{c}{Stay-at-home (March 16 - March 29, 2020)}\\
        \midrule
        % HomoG-GCN & 253 & 0.224 & 60.15 & 100\% & 3.79 & 482\% \\
        % Pois-GCN & 267.7 & 0.409 & 5.046 & 60.6\% & 4.91 & 624\% \\
        HetG-GCN & 161.3 & 0.251 & \textbf{9.266} & \textbf{93.1\%} & \textbf{3.38} & \textbf{429\%} \\
        TG-GCN & \textbf{144.5} & \textbf{0.145} & 13.07 & 97.4\% & 3.49 & 443\% \\
        Lap-GCN & inf & 0.242 & 10.42 & 91.4\% & 4.16 & 529\% \\
        GEns-GCN & inf & 0.319 & 12.86 & 88.4\% & 4.67 & 593\% \\
        % MC-GCN & -1 & -1.000 & 4.951 & 6.92\% & 5.53 & 703\% \\
        \midrule
        \midrule
        \multicolumn{7}{c}{Initial Recovery (June 8 - June 21, 2020)}\\
        \midrule
        % HomoG-GCN & 252.4 & 0.201 & 60.39 & 100\% & 2.76 & 66.3\% \\
        % Pois-GCN & 166.4 & 0.158 & 7.159 & 84\% & 2.86 & 68.6\% \\
        HetG-GCN & 170 & 0.077 & 10.41 & 92.9\% & 2.64 & 63.3\% \\
        TG-GCN & \textbf{141.5} & 0.055 & \textbf{11.75} & \textbf{94.4\%} & \textbf{2.62} & \textbf{62.7\%} \\
        Lap-GCN & inf & \textbf{0.050} & 11.07 & 92.2\% & 2.68 & 64.3\% \\
        GEns-GCN & inf & 0.102 & 11 & 92.9\% & 2.71 & 64.9\% \\
        % MC-GCN & -1 & -1.000 & 5.146 & 26.1\% & 4.07 & 97.6\% \\
        \midrule
        \midrule
        \multicolumn{7}{c}{Steady Recovery (Oct 12 - Oct 25, 2020)}\\
        \midrule
        % HomoG-GCN & 253.6 & 0.184 & 64.03 & 99.9\% & 4.23 & 50\% \\
        % Pois-GCN & 205 & 0.131 & 9.394 & 77.5\% & 4.24 & 50.1\% \\
        HetG-GCN & 177 & \textbf{0.057} & 15.23 & 89.3\% & \textbf{4.04} & \textbf{47.8\%} \\
        TG-GCN & \textbf{163.6} & 0.066 & 16.19 & 90.7\% & \textbf{4.04} & \textbf{47.8\%} \\
        Lap-GCN & 174 & \textbf{0.057} & \textbf{16.25} & \textbf{91.2\%} & 4.07 & 48.1\% \\
        GEns-GCN & 178.2 & 0.065 & 15.19 & 89.6\% & \textbf{4.04} & \textbf{47.8\%} \\
        % MC-GCN & -1 & -1.000 & 5.147 & 20.7\% & 5.69 & 67.3\% \\
        \midrule
    \end{tabular}
    }
    \label{tab:model_perf_tnc_test}
\end{table*}


% \begin{table*}[ht]
%     \centering
%     \caption{Model Generalizability}
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{c|c|c|c|c|c|c|c}
%         \toprule
%         Train Set & Test Set & Model & Negative LogLikelihood & Calibration Error & MPIW & PICP & MAE\\
%         \midrule
%         \multicolumn{8}{l}{\textbf{Panel 1: Train and test on the same dataset}} \\
%         \midrule
%         \textbf{Post} & \textbf{Post} & \textbf{HetG-GCN} & \textbf{70.89} & \textbf{0.056} & \textbf{75.31} & \textbf{95.7\%} & \textbf{13.14} \\
%         Post & Post & HetG-GAT & 71.09 & 0.015 & 71.19 & 95.4\% & 13.57 \\
%         \midrule
%         Post & Post & Lap-GCN & 71.32 & 0.025 & 77.27 & 97.0\% & 13.71 \\
%         Post & Post & Lap-GAT & 71.29 & 0.023 & 83.38 & 97.3\% & 13.53  \\
%         \midrule
%         \midrule
%         \multicolumn{8}{l}{\textbf{Panel 2: Train and test on the different datasets}} \\
%         \midrule
%         Pre & Post & HomoG-GCN & 102.68 (+44.8\%) & 0.194 (+246\%) & 302.02 & 100\% & 14.53 (+10.6\%)\\
%         Pre & Post & HetG-GCN & 74.02 (+4.41\%) & 0.096 (+71.4\%) & 102.35 & 99\% & 14.64 (+11.4\%)\\
%         Pre & Post & GEns-GCN & 73.31 (+3.41\%) & 0.088 (+57.1\%) & 97.72 & 99\% & 14.30 (+8.83\%) \\
%         Pre & Post & Lap-GCN & 72.84 (+2.75\%) & 0.075 (+33.9\%) & 114.80 & 100\% & 13.74 (+4.57\%)\\
%         \midrule
%         Pre & Post & HomoG-GAT & 102.76 (+45.0\%) & 0.185 (+230\%) & 301.53 & 100\% & 16.12 (+22.7\%)\\
%         Pre & Post & HetG-GAT & 74.85 (+5.59\%) & 0.117 (+109\%) & 97.28 & 98\% & 15.68 (+19.3\%)\\
%         Pre & Post & GEns-GAT & 73.66 (+3.91\%) & 0.091 (+62.5\%) & 96.65 & 99\% & 14.14 (+7.61\%)\\
%         Pre & Post & Lap-GAT & 72.76 (+2.64\%) & 0.070 (+25.0\%)& 111.95 & 99\% & 13.82 (+5.18\%) \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:model_robust_test}
% \end{table*}


% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%
\begin{comment}
\appendices
\section{Selection of Model Parameters}\label{appendix1}
Figure \ref{fig:lookback_select} shows the distribution of model performances from different lookback periods. Since different metrics are of different units, the y-axis is normalized by the overall mean performance for each data set to make the different metrics comparable. In both data sets, neither of the lookback choices show strict performance dominance. A lookback period of 2 exhibits the least variance in different model trainings, and therefore lookback period of 2 hours is chosen.

\begin{figure}
    \centering
    \subfloat[]{\includegraphics[width=\linewidth]{lookback_before.png}}\\
    \subfloat[]{\includegraphics[width=\linewidth]{lookback_after.png}}
    \caption{Performance w.r.t. Lookback Period (a) Before COVID-19, (b) During COVID-19}
    \label{fig:lookback_select}
\end{figure}


\end{comment}
% use section* for acknowledgment
\section*{Acknowledgment}

This material is based upon work supported by the U.S. Department of Energy’s Office of Energy Efficiency and Renewable Energy (EERE) under the Vehicle Technology Program Award Number DE-EE0009211. The views expressed herein do not necessarily represent the views of the U.S. Department of Energy or the United States Government. The authors would also like to thank the Chicago Transit Authority for providing access to public transit ridership data.


\bibliography{references}

